Bayesian hierarchical modelling for inferring genetic interactions in yeast

Identifying genetic interactions for a given microorganism such as yeast is difficult. Quantitative Fitness Analysis (QFA) is a high-throughput experimental and computational methodology for quantifying the fitness of microbial cultures. QFA can be used to compare between fitness observations for different genotypes and thereby infer genetic interaction strengths. Current "naive" frequentist statistical approaches used in QFA do not model between-genotype variation or difference in genotype variation under different conditions. In this thesis, a Bayesian approach is introduced to evaluate hierarchical models that better reflect the structure or design of QFA experiments. First, a two-stage approach is presented: a hierarchical logistic model is fitted to microbial culture growth curves and then a hierarchical interaction model is fitted to fitness summaries inferred for each genotype. Next, a one-stage Bayesian approach is presented: a joint hierarchical model which does not require a univariate summary of fitness, used to pass information between models. The new hierarchical approaches are then compared using a dataset examining the effect of telomere defects on yeast. By better describing the experimental structure, new evidence is found for genes and complexes which interact with the telomere cap. Various extensions of these models, including models for data transformation, batch effects, and intrinsically stochastic growth models are also considered.

==> Makefile <==
OBJECT= thesis
SOURCES		= $(OBJECT).tex \
references.bib  \
sections/abstract.tex sections/acknowledge.tex \
		  sections/introduction.tex \
		  sections/models.tex \
		  sections/SDE_approach.tex \
		  sections/case_studies.tex \
		  sections/appendix.tex \
	  sections_SDE/appendix.tex \
	  	  sections_SDE/application.tex \
	  	  sections_SDE/introduction.tex \
	  	  sections_SDE/LNAA.tex \
	  	  sections_SDE/LNAM.tex \
	  	  sections_SDE/Roman.tex \

ROBJECT= response
RSOURCES		= $(ROBJECT).tex \
references.bib  

LATEX=pdflatex

BIBTEX=bibtex

default=redraft.dvi


DEFAULT:
	make $(OBJECT).pdf

$(OBJECT).dvi: Makefile $(SOURCES)
	$(LATEX)  $(OBJECT)
	$(BIBTEX) $(OBJECT)
	makeindex $(OBJECT).nlo -s nomencl.ist -o $(OBJECT).nls
	$(LATEX)  $(OBJECT)
	$(LATEX)  $(OBJECT)

$(OBJECT).ps: $(OBJECT).dvi
	dvips $(OBJECT)

$(OBJECT).pdf: $(OBJECT).ps
	ps2pdf $(OBJECT).ps
	
response:
	make $(ROBJECT).pdf

$(ROBJECT).dvi: Makefile $(RSOURCES)
	$(LATEX)  $(ROBJECT)
	$(BIBTEX) $(ROBJECT)
	$(LATEX)  $(ROBJECT)
	$(LATEX)  $(ROBJECT)

$(ROBJECT).ps: $(ROBJECT).dvi
	dvips $(ROBJECT)

$(ROBJECT).pdf: $(ROBJECT).ps
	ps2pdf $(ROBJECT).ps

evince: $(OBJECT).pdf
	evince $(OBJECT).pdf

view: $(OBJECT).pdf
	acroread $(OBJECT).pdf
	
commit:
	svn commit
	make update

update:
	svn update
	svn log|less

clean:
	rm -f *.aux  *.nav *.out *.snm *.toc *.blg *.end *.log *~ *.nlo *.ist *.nls *.tmp sections/*.aux sections/*.tmp

pristine:
	make clean
	rm -f *.bbl $(OBJECT).pdf $(OBJECT).ps $(OBJECT).dvi
	rm -f *.bbl $(ROBJECT).pdf $(ROBJECT).ps $(ROBJECT).dvi



==> tables/SDE_diag_convergence.tex <==
\begin{table}[h!]
\caption{\label{app:sde_gia_con}Bayesian model convergence statistics for observed yeast data in Figure~\ref{real}}
\centering
\resizebox{\columnwidth}{!}{%
\npdecimalsign{.}
\nprounddigits{2}
\begin{tabular}{c c c c}
\hline
\emph{Model} & \emph{Parameter} & \emph{Effective Sample Size}  & \emph{Heidelberg and Welch P-value} \\ 
\hline
\cite{roman} & $\hat{K_p}$ & 1000 & 0.23 \\ 
     & $\hat{r_p}$ & 849 & 0.66\\ 
     & $\hat{P}$ & 1000 & 0.51\\
		& $\hat{\zeta}$ & 1099 & 0.91 \\
		 & $\hat{\nu}$ & 1000 & 0.17 \\
		LNAM & $\hat{K_p}$ & 1000 & 0.12\\
     & $\hat{r_p}$ & 1000 & 0.25 \\ 
     & $\hat{P}$ & 1000 & 0.21\\
		     & $\hat{\zeta}$ & 1075 & 0.91\\
	 & $\hat{\nu}$ & 987 & 0.38\\
		LNAA & $\hat{K_p}$ & 1000 & 0.11\\
     & $\hat{r_p}$ & 1000 & 0.25 \\ 
     & $\hat{P}$ & 1000 & 0.21\\
		     & $\hat{\zeta}$ & 1075 & 0.91\\
	 & $\hat{\nu}$ & 967 & 0.38\\				
\hline
\end{tabular}
\npnoround%
}
\end{table}













==> tables/SDE_values_bk.tex <==
\begin{table}[h!]
\caption{\label{tab:real_par} Bayesian model parameter posterior means, standard deviations and true values for Figure~\ref{self}}
\centering
\resizebox{\columnwidth}{!}{%
\npdecimalsign{.}
\nprounddigits{3}
\begin{tabular}{c c n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3}}
\hline
\emph{Figure~\ref{self} panel} & \emph{Model} & \multicolumn{2}{c}{\emph{$\hat{K}$}}  & \multicolumn{2}{c}{\emph{$\hat{r}$}}  & \multicolumn{2}{c}{\emph{$\hat{P}$}}  & \multicolumn{2}{c}{\emph{$\hat{\nu}$}} & \multicolumn{2}{c}{\emph{$\hat{\zeta}$}} \\ 
\hline
\noalign{\vskip 0.2mm} 
A & \cite{roman} & 0.14919 &(0.00308)& 3.00089 &(0.00963)& 9.95211e-05 &(7.968471e-07
)& 0.00500 &(0.00177)& 0.01084 &(0.00434)\\ 
B &  & 0.11147 &(0.00894)& 4.06539 &(0.04718)& 4.81416e-05 &(1.525998e-06)& 0.01063 &(0.00745)& 0.04891 &(0.01528)\\
C &  & 0.3004265 &(0.007933814)& 6.013413 &(0.02967878)& 0.0002000386 &(3.58488e-06)& 0.009867945 &(0.00354592)& 0.0174254 &(0.009317025)\\
A & LNAM & 0.14987 &(0.0003233746)& 2.99402 &(0.0086)& 9.95277e-05 &(7.609211e-07)& 0.00381 &(0.00166)& 0.01017 &(0.00482)\\ 
B &  & 0.11117 &(0.00067)& 3.96618 &(0.04231)& 4.97933e-05 &(1.417227e-06)& 0.00493 &(0.00425)& 0.04756 &(0.00952)\\ 
C &  & 0.3004188 &(0.000865403)& 6.025081 &(0.03846942)& 0.0001957017 &(4.1981e-06)& 0.007026462 &(0.003905458)& 0.02819256 &(0.01337349)\\ 
A & LNAA & 0.14960 &(0.00203)& 3.11276 &(0.28946)& 8.79417e-05 &(6.335433e-05)& 0.00581 &(0.00096)& 0.03934 &(0.02880)\\ 
B & & 0.11026 &(0.00071)& 3.98863 &(0.15093)& 5.08313e-05 &(1.359647e-05)& 0.00112 &(0.0004387244)& 0.04659  &(0.01845)\\
C & & 0.3009646 &(0.003118113)& 5.14457 &(0.4901047)& 0.0006172978 &(0.0003648014)& 0.00951418 &(0.002776264)& 0.05970999  &(0.04777153)\\
\\
\hline
\emph{Figure~\ref{self} panel} & & \multicolumn{2}{c}{\emph{K}} & \multicolumn{2}{c}{\emph{r}}  & \multicolumn{2}{c}{\emph{P}}   & \multicolumn{2}{c}{\emph{$\nu$}} & \multicolumn{2}{c}{\emph{$\zeta$}}\\ 
\hline
True Values for A, B and C &  & \multicolumn{2}{c}{0.15} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{0.0001} & \multicolumn{2}{c}{0.005} & \multicolumn{2}{c}{0.01} \\ 
True values for D, E and F & & \multicolumn{2}{c}{0.11} & \multicolumn{2}{c}{4} & \multicolumn{2}{c}{0.00005} & \multicolumn{2}{c}{0.001} & \multicolumn{2}{c}{0.05}  \\
True values for G, H and I & & \multicolumn{2}{c}{0.3} & \multicolumn{2}{c}{6} & \multicolumn{2}{c}{0.0002} & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.02}  \\
Parameter values for Figure~\ref{4nonu} simulations & & \multicolumn{2}{c}{0.11} & \multicolumn{2}{c}{4} & \multicolumn{2}{c}{0.00005} & \multicolumn{2}{c}{N/A} & \multicolumn{2}{c}{0.05}  \\
\hline
\end{tabular}
\npnoround%
}


\end{table}













==> tables/SDE_values_further_bk.tex <==
\begin{table}[h!]
\caption{\label{app:sde_val_fur}Bayesian model parameter posterior means, standard deviations and true values for Figure \ref{simlog}, \ref{sim} and \ref{real}}.
True values for the simulated data used for Figure \ref{simlog} and \ref{sim} are also given.
\centering
\resizebox{\columnwidth}{!}{%
\npdecimalsign{.}
\nprounddigits{3}
\begin{tabular}{c c n{2}{5} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3} n{1}{3}}
\hline
\emph{Dataset} & \emph{Model} & \multicolumn{2}{c}{\emph{$\hat{K}$}}  & \multicolumn{2}{c}{\emph{$\hat{r}$}}  & \multicolumn{2}{c}{\emph{$\hat{P}$}} & \multicolumn{2}{c}{\emph{$\hat{\nu}$}} & \multicolumn{2}{c}{\emph{$\hat{\zeta}$}}  \\ 
\hline
\noalign{\vskip 0.2mm} 
Simulated with Lognormal error  & \cite{roman} & 0.149999335 &(0.00341)&
2.99015285 &(0.01092)&
9.93119e-05 &(1.06863e-06)&
0.0056843212256 &(0.00236)&
0.011547265557 &(0.00618)\\ 
 & LNAM & 0.149614787 &(0.0004717042)&
2.98773783 &(0.01318)&
9.97960e-05 &(1.124219e-06)&
0.0041396496436 &(0.00217)&
0.016364920984 &(0.00517)\\
 & LNAA & 0.14953488 &(0.0005)&
3.00514737 &(0.01995)&
9.64713e-05 &(2.945503e-06)&
3.098832e-05 &(0.00002)&
0.0194997429 &(0.00344)\\ 
Simulated with Normal error  & \cite{roman} & 0.2127014398 &(0.12323)&
1.367943557 &(0.26339)&
0.00455 &(0.00211)&
0.25392518626 &(0.10969)&
0.41885683478 &(0.12943)\\ 
 & LNAM & 0.1714519199 &(0.03280)&
1.579950397 &(0.27107)&
0.00524 &(0.00204)&
0.205421122203 &(0.07805)&
0.4730700594  &(0.05100)\\ 
& LNAA & 0.150452393 &(0.00222)&
2.99999791 &(0.26239)&
1.189e-04 &(7.098716e-05)&
0.00549023564 &(0.00106)&
0.052829431599  &(0.03326)\\
Observed yeast data & \cite{roman} &  0.1143094 &(0.02602507)&
3.763728 &(0.2006525)&
1.079002e-05 &(3.154911e-06)&
0.3378525 &(0.04839998)&
0.07771955 &(0.07732242)\\ 
 & LNAM & 0.1103702 &(0.01113706)&
3.776766 &(0.216272)&
1.077129e-05 &(3.277218e-06)&
0.336179 &(0.05137415)&
0.1036413 &(0.1079923)\\
 & LNAA & 0.109176 &(0.003306315)&
3.832318 &(0.1984635)&
1.068951e-05 &(3.680477e-06)&
0.0001768693 &(6.606697e-05)&
0.1637506 &(0.03259627)\\
\\ 
\hline
\emph{Dataset} & & \multicolumn{2}{c}{\emph{K}}  & \multicolumn{2}{c}{\emph{r}}  & \multicolumn{2}{c}{\emph{P}} & \multicolumn{2}{c}{\emph{$\nu$}} & \multicolumn{2}{c}{\emph{$\zeta$}}   \\
\hline
\multicolumn{2}{c}{True values for simulated Lognormal and Normal datasets}  & \multicolumn{2}{c}{0.15} & \multicolumn{2}{c}{3} & \multicolumn{2}{c}{0.0001} & \multicolumn{2}{c}{0.005} & \multicolumn{2}{c}{0.01} \\ 
\hline
\end{tabular}
\npnoround%
}
\end{table}




